$k$-Universality of Regular Languages

A subsequence of a word $w$ is a word $u$ such that $u = w[i_1] w[i_2] \dots w[i_{k}]$, for some set of indices $1 \leq i_1 < i_2 < \dots < i_k \leq \lvert w\rvert$. A word $w$ is $k$-subsequence universal over an alphabet $\Sigma$ if every word in $\Sigma^k$ appears in $w$ as a subsequence. In this paper, we study the intersection between the set of $k$-subsequence universal words over some alphabet $\Sigma$ and regular languages over $\Sigma$. We call a regular language $L$ \emph{$k$-$\exists$-subsequence universal} if there exists a $k$-subsequence universal word in $L$, and \emph{$k$-$\forall$-subsequence universal} if every word of $L$ is $k$-subsequence universal. We give algorithms solving the problems of deciding if a given regular language, represented by a finite automaton recognising it, is \emph{$k$-$\exists$-subsequence universal} and, respectively, if it is \emph{$k$-$\forall$-subsequence universal}, for a given $k$. The algorithms are FPT w.r.t.~the size of the input alphabet, and their run-time does not depend on $k$; they run in polynomial time in the number $n$ of states of the input automaton when the size of the input alphabet is $O(\log n)$. Moreover, we show that the problem of deciding if a given regular language is \emph{$k$-$\exists$-subsequence universal} is NP-complete, when the language is over a large alphabet. Further, we provide algorithms for counting the number of $k$-subsequence universal words (paths) accepted by a given deterministic (respectively, nondeterministic) finite automaton, and ranking an input word (path) within the set of $k$-subsequence universal words accepted by a given finite automaton.

==> compmodel.tex <==
The computational model we use is the standard unit-cost RAM with logarithmic word size: for an input of size $n$, each memory word can hold $\log (n)$ bits. Arithmetic and bitwise operations with numbers in $[1,n]$ are, thus, assumed to take $O(1)$ time. Numbers larger than $n$, with $\ell$ bits, are represented in $O(\ell/\log n)$ memory words, and working with them takes time proportional to the number of memory words on which they are represented. In all the problems, we assume that we are given a number $k$, binary encoded, and one finite automaton $\mathcal A$, specified as the set of states, set of input letters, set of transitions, and initial and final states. The size of the input is, as such, the size of the binary encoding of $k$, which is $\lceil\log_2 k\rceil$, plus the size $S$ of the encoding of $\mathcal A$ (which is lower bounded by the number of edges in the graph associated to the automaton). So, one memory word can hold $\log (S+\log_2 (k))$ bits.\\
For a more detailed general discussion on this model see, e.\,g.,~\cite{crochemore}. 


%
%\begin{remark}
%	Note that both algorithms given in Theorems~\refl{thm:ESUPFA} and~\label{thm:ASUPFA} are fixed parameter tractable (FPT) algorithms w.r.t. $\sigma$ (and their run-time is polynomial for $\sigma\in O(\log n)$). Moreover, their time complexity does not depend at all on $k$.
%\end{remark}



==> general.tex <==
\begin{itemize}
\item Counting the $k$-universal words of a given NFA/DFA
\item What is the maximal $k$ such that $\mathcal{A}$ is $k$-universal
\item regular expressions for $k$-universal words
\item universality of the prefix/suffix automata
\item connection between suffix arrays and $k$-universality
\end{itemize}


\begin{proposition}
Given a regular language $L\subseteq\Sigma^{\ast}$ as regular expression $r\in(\Sigma\cup\{(,),|,\ast\})^{\ast}$, we can determine the universality indices of $L$'s shortest words in time $\mathcal{O}(|r|)$.
\end{proposition}

\begin{proof}
First, we determine $L$'s shortest words from $r$ by deleting all Kleene parts of $r$. Therefore, we maintain a stack $S$.
Set $r'=\varepsilon$.
Now, we read $r$ from left to right. Let $i\in[r]$. If $S=\emptyset$ and $w[i]\in\Sigma\cup\{|\}$ then append $w[i]$ to $r'$. Whenever, we have $w[i]=($, we push $i$ on $S$. If we read $w[j]=)$, we pop the associated $($ from $S$. Thus, $r'$ does not contain the Kleene star anymore and we have $|r'|\leq|r|$ with $r'$ being of the form $r_1|r_2|\cdots|r_k$ for some $k\in\N_0$ and $r_i\in\Sigma^{\ast}$ for all $i\in[k]$. In a second step, we go over $r'$ and determine the shortest words of $L$. We have a list $\ell$, where $\ell[i]$ stores all words of length $i$ in $L(r')$: read $r'$ from left to right and for each $r_j$ copy the word into a variable $x$, count $r_j$'s letters and add $r_j$ to $\ell(|x|)$. Since the largest index of $\ell$ cannot be larger than $|r|$, we can access the smallest $i$ with $\ell[i]\neq\emptyset$. For each such $i$, we can determine $\iota(r_i)$ in time $\mathcal{O}(|r_i|)$. Since $\sum_{i\in[k],|r_i|\mbox{ min}}|r_i|\leq|r'|$, we remain in $\mathcal{O}(|r|)$.
\end{proof}


==> proofs/ESUPFA_solving.tex <==
\begin{proof}
    From Lemma \ref{lem:ksu_min_length}, if there exists some $k$-universal word accepted by $\mathcal{A}$, there must exist some $k$-universal word of length at most $k n \sigma$.
    Using Corollary \ref{col:counting_up_to_ell_k_subsequence_univeral_words}, the number of $k$-universal words accepted by $\mathcal{A}$ of length at most $k n \sigma$ can be computed in $O(n^4 k^3 \sigma^3 2^{\sigma})$ time.
    By checking if there exists some $k$-universal word of length at most $k n \sigma$, the $k$-ESUPFA problem can be solved in $O(n^4 k^3 \sigma^3 2^{\sigma})$ time.
\end{proof}


==> proofs/NP_hard_1_universal.tex <==
\begin{proof}
	Let $G = (V, E)$ be a graph with $V = \{v_1, v_2, \dots, v_n\}$.
	
	An automaton $\mathcal{A}$ is constructed from $G$  as follows over the alphabet $\Sigma = \{1, 2, \dots n\}$. 
	Let $Q = \{q_{i,j} \mid i,j \in [n]\} \cup \{q_0, q_f\}$ where the last two states indicate the initial state and a failure state. The set of accepting states is given by $F = \{q_{n,j} \mid j \in [n]\}$.
	% Informally, the state $q_{i,j}$ is used to represent visiting vertex $v_j$ at the $i^{th}$ step of some path. 
	Now, we define the transition function $\delta : Q \times \Sigma \to Q$ by 
	\begin{align*}
		\delta(q, x) = 
		\begin{cases} 
			q_{i+1,\ell}, & \text{if } q = q_{i,j}, x = \ell, i < n, \text{ and } (v_j,v_\ell) \in E,\\
			q_f, & \text{if }  q=q_{i,j}\text{ and } (v_j,v_x) \not\in E,\\
			q_{1,x}, & \text{if } q = q_0,\\
			q_f & \text{if } q = q_{n, i}.
		\end{cases}
	\end{align*}
	Thus, the set of transition from each state $q_{i,j}$ represents the edges in $G$ incident to $v_j$. Each transition is labelled by the end vertex of the edge, i.e., the vertex that is reached after following the edge. Since $\mathcal{A}$ has $n^2+2$ states, $\mathcal{A}$ is constructible in polynomial time.
	
	
	%\bigskip
	
	Using this construction, observe that any word accepted by $\mathcal{A}$ corresponds to a path in $G$ of length $n$. Therefore, a Hamiltonian path can exist in $G$ if and only if there exists some word of length $n$ containing each symbol from $\Sigma$ exactly once. In other words, a Hamiltonian path exists in $G$ if and only if $\mathcal{A}$ contains a $1$-universal word. 
	% In the other direction, if a Hamiltonian path exists in $G$, a $1$-universal word exists in $\mathcal{A}$ corresponding to the Hamiltonian path. Similarly, if no such path exists, then no $1$-universal word can exist in $\mathcal{A}$. 
	Hence it is NP-hard to determine if at least one word accepted by $\mathcal{A}$ is $k$-universal, even for $k = 1$.
\end{proof}

==> proofs/counting_perfect_universal_paths.tex <==
\begin{proof}
	This can be achieved by determining the value of $U[q, \ell]$ by $U[q, \ell] \sum_{x \in \Sigma, q' \in \Delta(q, x)} T[q', \ell - 1, k - 1, \Sigma \setminus \{\tx\}]$, thus discarding any perfect $k$-universal paths of length $\ell - 1$.
\end{proof}


==> proofs/direct_paths_sufficent_every_word.tex <==
\begin{proof}
	% Assume first, that every word recognised by $\mathcal{A}$ is $k$-subsequence universal. 
	% Note that there must exist at least one non-cyclic path in $\mathcal{A}$. % Thus by assumption the words associated with the paths are $k$-subsequence universal as such the paths.
	% For the other direction, assume that every non-cyclic accepting path is $k$-subsequence universal. 
	In one direction, if $\mathcal{A}$ accepts any path that is not $k$-universal,  then not every path recognised by $\mathcal{A}$ is $k$-universal.
	Otherwise,  the set of paths induced by every word recognised by $\mathcal{A}$ must contain, as a subsequence, some non-cyclic path.
	Therefore, if each non-cyclic path is $k$-universal, then every path is.
	% Since, every word induced by a non-cyclic accepting path is $k$-subsequence universal, then every word recognised by $\mathcal{A}$ is $k$-subsequence universal.
\end{proof}

==> proofs/esupfa_decision.tex <==
The computational model we use is the standard unit-cost RAM with logarithmic word size: for an input of size $n$, each memory word can hold $\log (n)$ bits. Arithmetic and bitwise operations with numbers in $[1,n]$ are, thus, assumed to take $O(1)$ time. Numbers larger than $n$, with $\ell$ bits, are represented in $O(\ell/\log n)$ memory words, and working with them takes time proportional to the number of memory words on which they are represented. In all the problems, we assume that we are given a number $k$, binary encoded, and one finite automaton $\mathcal A$, specified as the set of states, set of input letters, set of transitions, and initial and final states. The size of the input is, as such, the size of the binary encoding of $k$, which is $\lceil\log_2 k\rceil$, plus the size $S$ of the encoding of $\mathcal A$ (which is lower bounded by the number of edges in the graph associated to the automaton). So, one memory word can hold $\log (S+\log_2 (k))$ bits.\\
For a more detailed general discussion on this model see, e.\,g.,~\cite{crochemore}. 


%
%\begin{remark}
%	Note that both algorithms given in Theorems~\refl{thm:ESUPFA} and~\label{thm:ASUPFA} are fixed parameter tractable (FPT) algorithms w.r.t. $\sigma$ (and their run-time is polynomial for $\sigma\in O(\log n)$). Moreover, their time complexity does not depend at all on $k$.
%\end{remark}



==> proofs/every_word_in_NP.tex <==
\begin{proof}
	% \todofpa{why is it $m^m$ and how is it for NFA?}
	From Lemma \ref{lem:direct_paths_sufficent_every_word}, every word recognised by $\mathcal{A}$ is $k$-universal if and only if every word induced by a non-cyclic path in $\mathcal{A}$ is $k$-universal. As any non-cyclic path may traverse at most one tranisition from any given state, the number of possible paths is at most $(\sigma + 1)^n$, where $n$ is the number of states in $\mathcal{A}$, as a path can be formed by chosing at most one of $\sigma$ transitions from each state.
	As every such path can be enumerated in $O(\sigma^n)$ time. Therefore $k$-ASUPFA is in co-NP.
\end{proof}


==> proofs/lem-asupfa.tex <==
\begin{proof}
Clearly, the set of words accepted by $\mathcal{A}$ which have the smallest universality index (among all words accepted by $\mathcal{A}$) includes a word which is the label of a simple path in $\mathcal{A}$. So, to solve the problem stated in this lemma it is enough to consider only words which are the label of simple paths in $\mathcal{A}$. The length of these words is upper bounded by $n$. This also shows that their universality index is upper bound by $n$ (so, as a consequence, this universality index and the numbers smaller than it fit in one memory word). 

	The solution of our problem is done by a dynamic programming algorithm. We define two $n\times 2^\sigma$ matrices $M, M'$ where initially $M[q][V]=M'[q][V]=\infty$ for $V\subseteq \Sigma$. Also, we use a set $L=\emptyset$. Further, set $M[q_0][\emptyset]=0$ and insert $(q_0,\emptyset)$ in $L$.
	
	We will maintain the property that before the \nth{$(r+1)$} iteration of our algorithm (for $r\geq 0$) $M[q][S]$ stores the minimal number of arches of the word $w_{r,q}$ of length at most $r$ which connects $q_0$ and $q$ such that $\letters(\r(w_{r,q})) = S$. This property clearly holds before the first iteration of the algorithm. 
	Now, we perform the following steps
\begin{lstlisting}[mathescape=true,backgroundcolor = \color{white}]
for $\ell = 1$ to $n$
  for all $(q,S) \in L$ 
    for all $a\in \Sigma$ and $q'\in \delta(q,\ta)$
      if $S\cup \{\ta\}=\Sigma$
        set $M'[q'][\emptyset]=M[q][S]+1$ and insert $(q',\emptyset)$ in $L$
      else 
        set $M'[q'][S\cup\{\ta\}]=M[q][S]$ and insert $(q',S\cup\{\ta\})$ in $L$
for all $q \in Q$ and $V\subseteq \Sigma$
  set $M[q][V]=\min\{M[q][V],M'[q][V]\}$
\end{lstlisting}
% 	\begin{algorithmic}
% 	\For{$\ell = 1$ to $n$}
% 		\ForAll{$(q,S) \in L$} 
% 			\ForAll{$a\in \Sigma$ and $q'\in \delta(q,\ta)$}
% 				\If{$S\cup \{\ta\}=\Sigma$}
% 					\State set $M'[q'][\emptyset]=M[q][S]+1$ and insert $(q',\emptyset)$ in $L$
% 				\Else 
% 					\State set $M'[q'][S\cup\{\ta\}]=M[q][S]$ and insert $(q',S\cup\{\ta\})$ in $L$
% 				\EndIf 
% 			\EndFor
% 		\EndFor
% 	\EndFor
% 	\ForAll{$q \in Q$ and $V\subseteq \Sigma$}
% 		\State set $M[q][V]=\min\{M[q][V],M'[q][V]\}$
% 	\EndFor
% 	\end{algorithmic}
% 	
	In the iteration of the outmost for-loop for $\ell=r$ we actually consider, for each pair $(q,S)$, the word $v$ of length at most $r-1$ which connects $q_0$ and $q$, such that $v$ has a minimum number of arches and $\letters(\r(v)) = S$ (the relevant information about this path, i.e., its rest and the number of arches is stored in $M$), and try to extend this path by one letter $\ta$. This leads to another pair $(q',S\cup\{\ta\})$, and we simply check if this is the word $v'$ with a minimum number of arches, of length at most $r$ which connects $q_0$ and $q'$, such that $\letters(\r(v'))$ is either $\emptyset$, when $\Sigma = S\cup\{\ta\}$, or $S\cup\{\ta\}$ otherwise (see also Lemma \ref{lem:making_a_path_longer}, which explains how a path is extended). This implies that the property which we wanted to maintain holds before the iteration of the loop for $\ell=r+1$. 
	
	The time complexity of this algorithm is $ O^*(n^3 2^\sigma)$.
	
	Now, the smallest universality index of a word accepted by $\mathcal{A}$ is simply the minimum entry $M[q][V]$, for a final state $q$.
\end{proof}


==> proofs/solving_existance.tex <==
\begin{proof}
    From Lemma \ref{lem:direct_paths_sufficent_every_word}, $\mathcal{A}$ can be universal $k$-universal if and only if every non-cyclic path is $k$-universal.
    Note that every non-cyclic path must have length at most $n$. 
    From Lemma \ref{col:counting_up_to_ell_k_subsequence_univeral_words} the number of $k$-universal words of length at most $n$ can be computed in $O(n^3 k \sigma 2^{\sigma})$ time.
    Similarly, the number of paths of length $\ell \in [1, n]$ in $\mathcal{A}$ ending at each state can be computed via classical techniques in $O(n^3)$ time, for every $\ell \in [1, n]$.
    By checking if the number of accepting paths of length at most $n$ matches with the number of accepted $k$-univseral words of length $n$,
    % As $\mathcal{A}$ is universal $k$-universal if and only if the number of paths of length at most $n$ ending at a final state is equal to the number of $k$-universal words of length at most $n$ recognised $\mathcal{A}$, 
    $k$-ASUPFA can be solved for $\mathcal{A}$ in $O(n^3 k  \sigma 2^{\sigma})$ time.
\end{proof}


==> proofs/thm-asupfa.tex <==
\begin{proof} 
We first use Lemma \ref{lem:ASUPFA} to compute $\ell$, the smallest universality index of a word accepted by $A$. If $\ell<k$, then the answer for the given instance of $k$-ASU is negative. Otherwise, the answer is positive.
\end{proof}

